Vision-by-Language for Training-Free Compositional Image Retrieval

Given an image and a target modification (e.g an image of the Eiffel tower and the text "without people and at night-time"), Compositional Image Retrieval (CIR) aims to retrieve the relevant target image in a database. While supervised approaches rely on annotating triplets that is costly (i.e. query image, textual modification, and target image), recent research sidesteps this need by using large-scale vision-language models (VLMs), performing Zero-Shot CIR (ZS-CIR). However, state-of-the-art approaches in ZS-CIR still require training task-specific, customized models over large amounts of image-text pairs. In this work, we propose to tackle CIR in a training-free manner via our Compositional Image Retrieval through Vision-by-Language (CIReVL), a simple, yet human-understandable and scalable pipeline that effectively recombines large-scale VLMs with large language models (LLMs). By captioning the reference image using a pre-trained generative VLM and asking a LLM to recompose the caption based on the textual target modification for subsequent retrieval via e.g. CLIP, we achieve modular language reasoning. In four ZS-CIR benchmarks, we find competitive, in-part state-of-the-art performance - improving over supervised methods. Moreover, the modularity of CIReVL offers simple scalability without re-training, allowing us to both investigate scaling laws and bottlenecks for ZS-CIR while easily scaling up to in parts more than double of previously reported results. Finally, we show that CIReVL makes CIR human-understandable by composing image and text in a modular fashion in the language domain, thereby making it intervenable, allowing to post-hoc re-align failure cases. Code will be released upon acceptance.

==> figs/teaser.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figs/teaser-v2.pdf}
    \caption{
    The task of Zero-Shot Composed Image Retrieval (ZS-CIR) has been approached by works that map an image to a single token. In contrast, we use off-the-shelf foundation models to generate a natural language description of the desired target image. This allows the user to clearly understand the overall process, especially since the natural language description of the target image is much more clear than a description that relies on the use of arbitrary tokens. 
    }
    \label{fig:teaser}
\vspace{-5pt}
\end{figure}

==> tables/captioning_comparison.tex <==
\begin{table}[t!]
    \centering
    \caption{Comparison of different publicly available SOTA captioning models on CIRCO validation show similar performance. \zeynep{the table above and this one can be combined into one tall table occupying space on the side of the paper. you can reduce the white space between columns}}
    \vspace{-6pt}    
    \resizebox{0.65\linewidth}{!}{
    \begin{tabular}{c|c|cccc}
    \toprule
     Arch & Method & mAP@5 & mAP@10 & mAP@25 & mAP@50\\
     \midrule
     ViT-B/32 & BLIP & 13.1 & 13.33 & 15.08 & 15.92\\
     ViT-B/32 & BLIP-2 & 13.33 & 14.16 & 15.74 & 16.35\\
     ViT-B/32 & CoCa & 13.64 & 13.37 & 15.10 & 15.90\\
    \bottomrule
    \end{tabular}}    
    \label{tab:captioning}
\vspace{-8pt}    
\end{table}


==> tables/cirr_comparison.tex <==
\begin{table}[t!]
    \centering
    \caption{\textbf{Comparison on CIRR Test Data.} Competitive results of \methodNameNS~against adaptive methods across this noisy benchmark offer further indication of efficacy. The simple scalability to very large retrieval models can provide further notable gains.  ($^*$) ViT-G/14 uses OpenCLIP weights.}
    \vspace{-8pt}
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{l|l|cccc|ccc}
    \toprule
     Arch & Method & R@1 & R@5 & R@10 & R@50 & $R_s$@1 & $R_s$@2 & $R_s$@3\\
     \midrule
     \multirow{3}{*}{ViT-B/32} & PALAVRA \citep{palavra} & 16.62 & 43.49 & 58.51 & 83.95 & 41.61 & 65.30 & 80.94\\
      & SEARLE \citep{searle} & 24.00 & 53.42 & 66.82 & 89.78 & 54.89 & 76.60 & 88.19 \\
      & \textbf{\methodNameNS} & 23.94 & 52.51 & 66.0 & 86.95 & 60.17 & 80.05 & 90.19 \\
    \midrule
     \multirow{3}{*}{ViT-L/14} & Pic2Word \citep{pic2word} & 23.90 & 51.70 & 65.30 & 87.80 & - & - & - \\
      & SEARLE \citep{searle} & 24.24 & 52.48 & 66.29 & 88.84 & 53.76 & 75.01 & 88.19\\
      & \textbf{\methodNameNS} & 24.55 & 52.31 & 64.92 & 86.34 & 59.54 & 79.88 & 89.69\\    
     \midrule
     ViT-G/14$^*$ & \textbf{\methodNameNS} & 34.65 & 64.29 & 5.06 & 91.66 & 67.95 & 84.87 & 93.21\\
    \bottomrule
    \end{tabular}}    
    \label{tab:cirr}
\vspace{-8pt}    
\end{table}

==> tables/genecis_evaluation.tex <==
\begin{table}[t]
%\footnotesize
\centering
\caption{\textbf{Evaluation on GeneCIS Test Data.} Methods using CIR triplets marked \gray{gray}. The competitive performance of \methodNameNS~across subtasks even against adapted baselines indicates its generality.
}
\vspace{-5pt}
\label{tab:genecis}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc|ccc|cc}
\toprule
& \multicolumn{3}{c}{Focus Attribute} & \multicolumn{3}{c}{Change Attribute} & \multicolumn{3}{c}{Focus Object} & \multicolumn{3}{c}{Change Object} \\
\cmidrule(rl){2-4}
\cmidrule(rl){5-7}
\cmidrule(rl){8-10}
\cmidrule(rl){11-13}
 &  R@1 & R@ 2 & R@3 & R@1 & R@ 2 & R@3 & R@1 & R@ 2 & R@3 & R@1 & R@ 2 & R@3 & Avg. R@1 \\
\midrule
Image Only        &  17.7       & 30.9       & 41.9 & 11.9       & 20.8       & 28.8 & 9.3       & 18.2       & 26.2 & 7.2       & 16.7       & 24.9   & 11.5    \\
Text Only         &  10.2       & 20.5       & 29.6 & 9.5       & 17.6       & 26.4 & 6.5       & 16.8       & 22.4 & 6.2       & 13.9       & 21.4    & 8.1   \\
Image + Text      &  15.6       & 26.3       & 37.1 & 12.6       & 22.9       & 32.0 & 10.8       & 21.0       & 31.2 & 11.3       & 21.5       & 30.3   & 12.6    \\
\gray{Combiner (CIRR)}      &  \gray{15.1}       &  \gray{27.7}       & \gray{39.8} & \gray{12.1}       & \gray{22.8}      & \gray{31.8} & \gray{13.5}       & \gray{25.4}       & \gray{36.7} &     \gray{15.4}   & \gray{28.0}       & \gray{39.6}   & \gray{14.0}    \\

\gray{Combiner (CC3M)}              &  \gray{19.0}       & \gray{31.0}       & \gray{41.5} & \gray{16.6} & \gray{27.5} & \gray{36.5} & \gray{14.7} & \gray{25.9}       & \gray{36.1} & \gray{16.8} & \gray{29.1} & \gray{39.7} & \gray{16.8}    \\  
\midrule
\textbf{\methodNameNS} & 17.9 & 29.4 & 40.4 & 14.8 & 25.8 & 35.8 & 14.6 & 24.3 & 33.3 & 16.1 & 27.8 & 37.6 & 15.9\\
\bottomrule
\end{tabular}
}
\vspace{-8pt}
\end{table}

==> tables/llm_comparison.tex <==
\begin{table}[t!]
    \centering
    \caption{Comparison between different LLMs on CIRCO validation reveals positive relation between peeformance and reasoning capacities.}
\vspace{-8pt}
    \resizebox{0.65\linewidth}{!}{
    \begin{tabular}{c|c|cccc}
    \toprule
     Arch & Method & mAP@5 & mAP@10 & mAP@25 & mAP@50\\
     \midrule
     ViT-B/32 & Captioning & 9.22 & 10.05 & 11.44 & 12.08\\
     ViT-B/32 & LLama2-70B & 10.22 & 10.60 & 11.80 & 12.39\\
     ViT-B/32 & Vicuna-13B & 12.65 & 13.17 & 14.48 & 15.20\\
     ViT-B/32 & GPT-3.5-Turbo & 13.33 & 14.16 & 15.74 & 16.35\\
     ViT-B/32 & GPT-4 & 15.63 & 16.31 & 17.02 & 18.12\\
    \bottomrule
    \end{tabular}}    
    \label{tab:llm}
\vspace{-8pt}
\end{table}

